Alopex: A Computational Framework for Enabling On-Device Function Calls with LLMs

The rapid advancement of Large Language Models (LLMs) has led to their increased integration into mobile devices for personalized assistance, which enables LLMs to call external API functions to enhance their performance. However, challenges such as data scarcity, ineffective question formatting, and catastrophic forgetting hinder the development of on-device LLM agents. To tackle these issues, we propose Alopex, a framework that enables precise on-device function calls using the Fox LLM. Alopex introduces a logic-based method for generating high-quality training data and a novel ``description-question-output'' format for fine-tuning, reducing risks of function information leakage. Additionally, a data mixing strategy is used to mitigate catastrophic forgetting, combining function call data with textbook datasets to enhance performance in various tasks. Experimental results show that Alopex improves function call accuracy and significantly reduces catastrophic forgetting, providing a robust solution for integrating function call capabilities into LLMs without manual intervention.

==> abstract.tex <==
\cite{frantar2023sparsegpt}

==> sections/futurework.tex <==
\section{Future Work}

This study contributes to the methodology of efficiently constructing a high quality function call dataset and addresses how to mitigate catastrophic forgetting during training in self-supervised learning. In the future, we would like to explore whether Fox can correctly generate output when there are variations in the parameters of function descriptions, a reduction in 10 function descriptions, and the addition of a completely new function description. Additionally, we want to investigate how to handle cases where the length of the input text exceeds the LLMs maximum context length.
